VisionKG: Unleashing the Power of Visual Datasets via Knowledge Graph

The availability of vast amounts of visual data with heterogeneous features is a key factor for developing, testing, and benchmarking of new computer vision (CV) algorithms and architectures. Most visual datasets are created and curated for specific tasks or with limited image data distribution for very specific situations, and there is no unified approach to manage and access them across diverse sources, tasks, and taxonomies. This not only creates unnecessary overheads when building robust visual recognition systems, but also introduces biases into learning systems and limits the capabilities of data-centric AI. To address these problems, we propose the Vision Knowledge Graph (VisionKG), a novel resource that interlinks, organizes and manages visual datasets via knowledge graphs and Semantic Web technologies. It can serve as a unified framework facilitating simple access and querying of state-of-the-art visual datasets, regardless of their heterogeneous formats and taxonomies. One of the key differences between our approach and existing methods is that ours is knowledge-based rather than metadatabased. It enhances the enrichment of the semantics at both image and instance levels and offers various data retrieval and exploratory services via SPARQL. VisionKG currently contains 519 million RDF triples that describe approximately 40 million entities, and are accessible at https://vision.semkg.org and through APIs. With the integration of 30 datasets and four popular CV tasks, we demonstrate its usefulness across various scenarios when working with CV pipelines.

==> 05useCases-backup.tex <==
\vspace{-6mm}
\section{Unified Access for Integrated Visual Datasets}
\label{sec:visionkg}
\vspace{-5mm}

 %The integration of data from different sources has been made possible by the flexible and powerful mechanism offered by Semantic Web technologies[]. However, the use of such technologies to manage computer vision (CV) datasets have been limited[]. Prominent CV datasets, such as ImageNet[] or Microsoft COCO[], only use a light form of taxonomy (e.g., WordNet[]) to label their images. Even when the subsets or samples from these datasets can be queried, the lack of a unified engine leads to an enormous workload that covers common possible use cases, such as querying samples under the same annotations from multiple datasets or unifying the labels across datasets.

% VisionKG addresses those issues by interlinking labels across label spaces(in interlinking the built-in datasets via knowledge graph technology) under shared semantic understanding, making it easy for users to use SPARQL to retrieve images that meet specific criteria, regardless of the complicated taxonomies across datasets. This is particularly useful for users who demand images of specific scenarios across multiple datasets under diverse tasks, such as pedestrian and vehicle detection in adverse weather conditions[] or occlusion-aware pose estimation[].

% To demonstrate the practical usefulness of our framework, we present three use cases that utilize VisionKG for exploring images and annotations with unified access through SPARQL queries, create composite visual datasets in a unified taxonomy across various tasks and sources, and how our system expedites the construction of pipelines for robust visual recognition systems based on VisionKG. Exploiting knowledge graph features paves the way to building supporting features for MLOPs in Section~\ref{VKG_MLOps}.

% As spotlighted in Section~\ref{Sec:VisionKG_FAIR}, the importance and challenges surrounding FAIR principles for visual datasets necessitate a comprehensive framework. 
In this Section, we first provide a detailed overview of the architecture of VisionKG, and discuss how it supports access to various popular visual datasets and computer vision tasks. We then demonstrate VisionKG's capabilities in providing unified access to integrated visual datasets via SPARQL queries, ultimately promoting and accelerating data streaming in CV pipelines. 
%%% This paves the way to building supporting practical usefulness of our framework for MLOps~\cite{alla2021mlops} in Section~\ref{Sec:VKG_MLOps} exploiting knowledge graph features.%%%
It shows practical usefulness of our framework for MLOps~\cite{alla2021mlops} in Section~\ref{Sec:VKG_MLOps} by exploiting knowledge graph features.


% \subsection{Building An Architecture to Facilitate Unified Access}\label{subsec:vkg_overview}
\subsection{VisionKG Architecture to Facilitate Unified Access}\label{subsec:vkg_overview}


% Figure~\ref{fig:visionkg-overview} illustrates our Vision Knowledge Graph (VisonKG)
% We collect images, annnotation form popular computer vision datasets such as Image
Figure~\ref{fig:visionkg-overview} provides an overview of our VisionKG framework and the process of creating and enriching our unified knowledge graph for visual datasets. We begin by collecting popular computer vision datasets that have significantly contributed to the development of visual recognition systems and extract their annotations and features across datasets using a \textit{Visual Extractor}.
\begin{figure}[ht!]
    \centering
    \includegraphics[width=\textwidth]{figures/[ISWC23] VIsionKG_Overview_DRAFT_v5.jpg}
    \caption{Overview of Vision-Knowledge-Graph (VisionKG) (\textcolor{red}{DRAFT})}
    \label{fig:visionkg-overview}
\end{figure}

% The design of VisionKG aims for genericity and reusability of visual datasets. For datasets from the same task, such as MS-COCO and VOC for object detection, VisionKG can quickly provide integrated support benefiting from the unified pre-defined metadata description. For datasets for distinct tasks VisionKG can also offer excellent scalability with cost-effective and consistent adaptations by benefiting from the well-designed schema.

% The search enrichment functionality in VisionKG focuses on providing users with their desired visual datasets consisting of images and annotations through a well-designed schema. Our framework supports the recombination and extension of knowledge retrieved from the knowledge graph. This enables an enriched functionality for multi-source datasets in VisionKG, satisfying individual user preferences. To elaborate further, for a dataset $D$ to be used for task $T$, containing subtasks $T_1$, $T_2$, $T_n$, e.g., both instance segmentation and semantic segmentation belong to image segmentation, the task can be converted from the queried source task to the target task by utilizing constraints, e.g. it can serve to convert the annotation of instance segmentation to semantic segmentation, thereby enriching the datasets. 


% Currently, our framework supports the following task-retrieval based on SPARQL: (i) single-source/multi-source data retrieval, (ii) single-task/multi-task retrieval, and (iii) task transformation, for instance, converting annotations of object detection to image classification. By querying single-source/tasks or multi-source/tasks data from VisionKG, users can execute different downstream pipelines, which can significantly reduce repetitive workload in the data processing.
% \textbf{add label convertor API, instance to semantic; detection to classification}

Next, to create a unified data model for the annotations and visual features, we follow the Linked Data principles~\cite{bizer2011linked} and use the RDF data model. Data entities such as images, boxes, and labels are named using Uniform Resource Identifiers (URIs). RDF data model, serving as a \textit{Semantic Annotator}, allows the data to be expressed using triples of the form $\langle \mathit{subject}, \mathit{predicate}, \mathit{object} \rangle$. For instance, to describe “an image contains a bounding box for a person" in MS-COCO~\cite{lin2014microsoft}, we assign unique URIs, e.g., \textit{vision.semkg.org/img01} and \textit{vision.semkg.org/box01}, for the image and the bounding box, respectively. Then, the following triples for such image with a box-level annotated {Person} can be described by the following triples: $\langle \mathit{image01}, \mathit{hasBox}, \mathit{box01} \rangle$ indicates that image has a box-level annotation, $\langle \mathit{box01}, \mathit{hasObject}, \mathit{obj01} \rangle$ describes that a box is an object, and $\langle \mathit{obj01}, \mathit{rdf:type}, \mathit{Person} \rangle$ point the object to the {Person}. In this way, the basic image-semantics pairs according to images and annotations can be constructed and then serve to analyze the structure of the collected CV datasets, which prepare to interlink these datasets.

Following FAIR principles described in Section~\ref{Sec:VisionKG_FAIR}, we add metadata to the integrated datasets, e.g., to describe what the entity is about and where it comes from. To enhance interoperability and enrich semantics in VisionKG, we also link the data with multiple knowledge bases, such as WordNet~\cite{Miller:1995} and Wikidata~\cite{nielsen2018linking}. These compose a \textit{Semantic Enrichment Reasoner} and ensure the reuse and enhance the taxonomy of the labels defined by the original sources. \textit{Semantic Enrichment Reasoner} expands the taxonomy by materializing the labels in each dataset using the ontology hierarchy, e.g.,  \verb|{pedestrian}| or \verb|{man}| \name{isSubClassOf}| \verb|{person}|. Based on the interlinked datasets and Semantic Enrichment Reasoner, we can build our unified knowledge graph. To ensure that interlinked datasets are accessible, we assign an endpoint to interface requests query and construct a SPARQL Engine to better process the queries across datasets with fruitful semantics.

Moreover, to ease the image query process and give users a quick view of the results, VisionKG offers a front-end web interface that allows users to explore queried datasets, such as visualizing data distribution and their corresponding annotations. The Lexical Similarity Module can prompt users if similar categories exist in other datasets, e.g., when users try to retrieve images with the \name{Person} from the MS-COCO dataset, they can also determine if images with \name{Pedestrian} and \name{Person\_Sitting} categories from the KITTI dataset should be included as supplementary results. Furthermore, our framework includes a DNN Training Engine, which contains many pre-trained models, such as FRCNN~\cite{ren2015faster} and YOLO-series~\cite{jiang2022review}. Based on those pre-trained models, VisionKG constructs an Evaluator, which gives users a quick overview of the quality of annotations. Users can also employ our pre-trained models to ensemble inference results and gain insights for subsequent practical training pipelines. Hence, VisionKG exploits features from knowledge graphs and visual datasets and ultimately serves as a comprehensive solution for users to access high-quality visual data and develop practical training pipelines with enriched semantics.

\subsection{Linked Datasets and Tasks in VisionKG}\label{subsec:vkg_linkedData}
Based on the architecture and schema of VisionKG demonstrated in Section~\ref{sec:inteop} and ~\ref{subsec:vkg_overview}, the current version of our framework (by May 2023) integrates thirty most common-used and popular visual datasets, involved in the tasks for visual relationship detection, image classification, object detection, and instance segmentation. Table~\ref{tab:Statistics} gives an overview of the contained datasets, images, annotations, and triples. In total, VisionKG encompasses over 519 million triples distributed among these tasks. 

\begin{table}[ht!]
\centering
\begin{tabular}{ccccc}
\toprule[0.8pt]
\textbf{Visual Tasks}                 &\textbf{\myhash Datasets} & \textbf{\myhash Images} & \textbf{\myhash Annotations} & \textbf{\myhash Triples} \\ \hline
Visual Relationship   & 2          & 119K          &1.2M               & 2.1M              \\
Instance Segmentation & 7          & 300K          &3.9M               & 22.4M               \\
Image Classification  & 9          & 1.7M          &1.7M               & 16.6M             \\
Object Detection      & 12         & 4.3M          &50.8M               & 478.7M               \\ \hline
Total                 & 30         & 6.4M          &57.6M               & 519.8M              \\
\bottomrule[0.8pt]
\end{tabular}
\caption{Statistics of VisionKG}
\label{tab:Statistics}
\end{table}

To enhance the effectiveness of our framework for image classification tasks, we have integrated both large benchmark datasets, such as ImageNet~\cite{deng2009imagenet}, as well as smaller commonly used datasets, like CIFAR~\cite{krizhevsky2009learning}, the diversity of covered datasets enables users to quickly and conveniently validate model performance, thus avoid extra laborious work. Table~\ref{tab:visionkg_classification} demonstrates that ImageNet comprises 1.2 million entities, dominating the distribution of the classification task in VisionKG. From linked relations across datasets and tasks, users can query different categories and the desired number of images to tailor training pipelines for specific scenarios. 
\begin{table}[ht!]
\centering
\begin{tabular}{lccccccc}
\toprule[0.8pt]
\multicolumn{1}{c}{}           & \textbf{IMN}   & \textbf{SOP} & \textbf{CIFAR} & \textbf{MNIST}  & \textbf{CART} & \textbf{Cars196} & \textbf{CUB200} \\ \hline
\myhash  Entities & 2.7M     & 240K      &
240K & 140K    & 77K     & 32.4K     & 23.6K    \\
\myhash  Triples  & 13.3M & 1.2M   & 1.2M   & 0.7M & 0.4M  & 0.2M  & 0.1M \\ 
\bottomrule[0.8pt]
\end{tabular}
\caption{Triples and Entities in VisionKG for Image Classification. IMN:ImageNet\cite{deng2009imagenet}, SOP: Stanford Online Products~\cite{oh2016deep},CIFAR:CIFAR10/100~\cite{krizhevsky2009learning}, CART: Caltech-101/-256~\cite{griffin2007caltech}, CUB200: Caltech-UCSD Birds-200-2011~\cite{wah2011caltech}.}
\label{tab:visionkg_classification}
\end{table}
For object detection, Table~\ref{tab:Statistics} and Table~\ref{tab:visionkg_detection} show that VisionKG comprises approximately 478 million triples for bounding boxes with dense annotations mainly contributed by large-scale datasets like OpenImages~\cite{kuznetsova2020open} and Objects365~\cite{shao2019objects365}. 
%This richness 
The variety of visual features allows users to create diverse mixed datasets based on their individual requirements for the size or the density of bounding boxes, which can be helpful to reduce biases solely introduced by a single dataset captured under specific conditions, e.g., to enhance the model performance on densely distributed small objects, which are typically challenging to localize and recognize~\cite{lin2017focal,lin2017feature}.
% In future work, we plan to explore and integrate more fine-grained relations between images and objects extending to more feature-fruitful datasets, such as V3DET and SA-1B. 
\begin{table}[ht!]
\centering
\begin{tabular}{lcccccccccc}
\toprule[0.8pt]
\multicolumn{1}{c}{} & \textbf{MSC}   & \textbf{UAD}  & \textbf{KIT}  & \textbf{CAR}  & \textbf{BDD}  & \textbf{OID}  & \textbf{O365} & \textbf{LVIS} & \textbf{MVD} & \textbf{VOC} \\ \hline
\myhash Entities           & 1.0M     & 678K    & 47K    & 32K    & 1.5M    & 14.3M    & 28.5M    & 1.6M    & 1.2M   & 138K   \\
\myhash Triples            & 9.7M & 6.4M & 0.4M & 0.3M & 15.1M & 135.8M & 277.4M & 15.9M    & 11.9M   & 1.0M   \\ 
\bottomrule[0.8pt]
\end{tabular}
\caption{Triples and Entities in VisionKG for Object Detection, MSC: MS-COCO\cite{lin2014microsoft}, UAD: UA-DETRAC~\cite{wen2020ua}, KIT: KITTI~\cite{geiger2013vision}, CAR: StanfordCars196~\cite{KrauseStarkDengFei-Fei_3DRR2013}, BDD: BDD100K~\cite{yu2020bdd100k}, OID: OpenImages~\cite{kuznetsova2020open}, O365: Objects365~\cite{shao2019objects365}, LVIS~\cite{gupta2019lvis}, MVD~\cite{neuhold2017mapillary}, VOC~\cite{Everingham10}}
\label{tab:visionkg_detection}
\end{table}
For visual relationship detection, which aims to recognize relationships between objects in images, we have further integrated datasets such as VisualGenome~\cite{krishna2017visual} and SpatialScene~\cite{yang2019spatialsense}, containing over 1.9 million triples for both bounding boxes and object-level relationships. Besides, VisionKG comprises 22.4 million triples for task instance segmentation, allowing users to retrieve and reuse masks of all instance-level objects for downstream scenarios, thus improving the pixel-level segmentation performance of models.
% VisionKG contains numerous entities and triples related to various visual tasks. To illustrate the distribution of datasets among various tasks, Figure \ref{fig:triple_entities} shows the number of triples and entities of each dataset per task. In Figure 5(a), ImageNet comprises 1.2 million entities, dominating the distribution of the classification task in VisionKG. As shown in Figure 5(b), the average number of triples per image in OpenImages and Objects365 is 10.2 and 13.6, respectively, indicating that more densely annotated objects appear in both datasets than others, for example, ..... This richness enables users to construct diverse mixed datasets according to their individual requirements based on the size or the density of bounding boxes, which can be helpful to address biases introduced by single-source datasets captured under specific conditions, e.g., to enhance the model performance on densely distributed small objects, which are typically difficult to localize and classify[].
% Figure 5(c) and 5(d) show the average number of triples per image from datasets used for instance segmentation and visual relationship detection.
\subsection{Visual Dataset Explorer powered by SPARQL}\label{sec:explorer}

\begin{figure}[ht!]
   \centering
   \includegraphics[width=1\textwidth]{figures/demo.drawio.png}
   \caption{VisionKG Demo}
   \label{fig:visionkg-demo}
\end{figure}

% As computer vision gains practical applications, datasets have become a crucial component in building visual learning pipelines that deliver high-performance models. Over the past decade, large-scale datasets such as ImageNet~\cite{deng2009imagenet}, OpenImages~\cite{kuznetsova2020open}, and Objects365~\cite{shao2019objects365} have been developed in the community. However, the taxonomy and annotation formats used by these datasets differ significantly. Hence, organizing training data from heterogeneous formats with distinct taxonomies in one pipeline is a time-consuming task for users of these datasets.

%%% As computer vision gains practical applications, %%%
As widely acknowledged, in practical applications of modern computer vision, datasets is a crucial component in building visual learning pipelines that deliver high-performance models. However, the taxonomy and annotation formats used by these datasets differ significantly. Hence, organizing training data from heterogeneous formats with distinct taxonomies in one pipeline is a time-consuming task for users of these datasets. 

Drawing from the architecture of VisionKG and integrated linked datasets introduced in Sections~\ref{subsec:vkg_overview} and ~\ref{subsec:vkg_linkedData},  to address the above problems, our framework provides a SPARQL interface to access, manage, and combine data efficiently exploiting the rich semantics of SPARQL. This enables users to describe their requirements or specific criteria using RDF statements. 
% For instance, if users want to extract images with bounding boxes of \verb|{car}| and \verb|{van}| from KITTI~\cite{geiger2013vision}, typically they would need to parse and iterate the corresponding annotation files, and then return the annotations which meet the user-defined requirements. Using VisionKG, users can conveniently query the desired images and their associated annotations using just a few lines of SPARQL. Figure~\ref{fig:UC1}\textbf{(a)} demonstrates how users can query images and annotations which meet the conditions mentioned in the example above. The possibility to use SPARQL enables users to construct scenario-specific datasets based on their specific use cases and conveniently alleviates extra workload in the aspects of data collection and preparation.
% \textcolor{red}{this part describe the demo}
For instance, our visual datasets explorer equipped with a live-interactive SPARQL interface is demonstrated in Figure~\ref{fig:visionkg-demo}. Users may begin by selecting a task, such as Detection, Classification, Segmentation, or Visual Relationship, from a menu \circled{1}. Once a task is chosen, the system will automatically generate a list of all available datasets that support the selected task \circled{2}.

Next, users may choose a dataset from the list, such as COCO or KITTI, and the system will display all available categories within that dataset \circled{3}. Users may conveniently filter categories by entering a keyword in a text box \circled{4}. This process is further enhanced by allowing users to drag and drop a category from \circled{3} to the SPARQL-query box \circled{6}. The system will automatically generate a SPARQL-query, along with explainable text \circled{5}, that selects images containing the specified category. It is noteworthy that multiple categories from different datasets can be selected. Users may modify the query by removing categories or changing the query conditions by selecting available options from box \circled{5}. Users may also adjust the number of images to be retrieved.

Once the query is finalized, the user may click the "Query" button, and the results will be displayed in table format \circled{7}. Additionally, users may select the "Visualization" tab \circled{8} to view the results graphically. By clicking on an image, users may access additional information, such as annotations of that image and annotations generated from popular deep learning models \circled{9}. Overall, the platform offers an intuitive and efficient method for dataset selection and querying for machine learning tasks.

% The possibility to use SPARQL enables users to construct scenario-specific datasets based on their specific use cases in a convenient fashion and allows them build robust training pipelines, as this reduces the bias arising from unrelated samples.

In advanced settings, as depicted in Figure~\ref{fig:UC1}\textbf{(b)}, users can also employ more fine-grained criteria for retrieving images with annotations, such as querying for ``images that contain a car captured during the night.'' This extends VisionKG's functionalities further for exploring and constructing datasets, allowing users to build models that cater for various scenarios more conveniently, e.g., samples with adverse weather conditions or samples collected at different times of the day. Additionally, for gaining a deeper understanding of the returned dataset, VisionKG offers a \textit{Evaluator} based on built-in models, and a web-based \textit{Visualizer}. In this way, users can explore and build their desired datasets tailored to their custom use cases with samples and desired annotations based on advanced query settings.
% from  create mixed-test datasets or subsets from diverse sources to construct the training pipeline and aim for a more robust model under various scenarios, such as adverse weather conditions or samples collected at different times of the day. For that, we describe a specific use case in Figure \ref{fig:UC1}. It shows how users can query for images of one category "car" from MS-COCO,  one category "car"  under rainy weather from BDD100K, and two categories "car" and "van" from KITTI using a simple query rather than a more complex query that covers all possible cases. In this way, users can construct a scenario-specific dataset based on their diverse use cases and build a more robust training pipeline against the bias resulting from the single-source dataset. In advanced settings, users can have more fine-grained criteria for retrieving images such as the query for "images that contain a car captured during the night", which enriches the potential of VisionKG for exploring/constructing datasets and help users to build models with various scenarios in a more convenient way. In addition, for quick verification of the retrieved images and to provide users with a deeper understanding of the dataset, VisionKG also provides built-in models to visualize the recognized results in time. Therefore, based on VisionKG, users can explore and build their desired datasets aiming to their customized use cases, then the VisionKG system will provide them with samples with desired annotations according to their query conditions.
\begin{figure}[ht!]
    \centering
    \includegraphics[width=\textwidth]{figures/UC/[ISWC23] VIsionKG_UC12.jpg}
    \caption{Dataset-Exploration with SPARQL under various conditions in VisionKG. }
    \label{fig:UC1}
\end{figure}
% \vspace{-5mm}
% \textbf{UC1-NOTE: need to add a figure with sparql to illustrate this subsec. }
% \textbf{We should highlight that the task can be done by writing a query rather than writing code. }
% Data exploring is one of the first task that the users usually ... 
% Before training a Neural Network, users usually need to discover labeled images. The data can be  diverse annotated structures and Tasks such as object detection and semantic segmentation, can be a time-consuming and repetitive process. 
% Users are typically required to obtain annotations from corresponding datasets and understand their formats before extracting desired annotations, which can vary significantly depending on the dataset. For instance, extracting a category instance labeled "car" from datasets like COCO, VOC, or KITTI involves parsing annotations from JSON or HTML formats while also considering different attributes and annotated structures. VisionKG addresses this challenge by providing a unified descriptor for different data formats based on knowledge graph, enabling users to easily query specific annotations from built-in datasets using the SPARQL query language.
% What we could sell:
% %\vspace{-2.5mm}
% \begin{enumerate}
%     \item parse annotations with diff. format, e.g. JSON, HTML, JPEG, which are time-consuming and not user-friendly
%     \item extract desired attributes/categories(datasets are separated and not linked together)
%     \item VisionKG can accelerate and facilitate it
%     \item user can query(similar to figure 1) \textbf{car}, \textbf{person} from single/multiple datasets for object detection, semantic segmentation, or even image classification
% \end{enumerate}
% % \vspace{5mm}
% \textbf{UC2. Integrating datasets from different sources into one unified space using VisionKG, e.g. wikidata, semantic web, wordNet,freebase:}
% \vspace{-5mm}

\section{VisionKG for MLOps}\label{Sec:VKG_MLOps}
% [one paragraph to give context : 1) link to first previous, 2) how use those feature, ] ... this section will demonstrate some popular features support MLOPs... due to space limit, we redirect readers to our git for more tutorials with notebooks...

% with ... above,... now we're ready to to carry nore complicated MLOps steps..., next...
The term \textit{MLOps} refers to the application of the DevOps process specifically for machine learning (ML), where model performance is primarily influenced by the quality of the underlying data~\cite{alla2021mlops}. As demonstrated in Section~\ref{sec:visionkg}, the detailed overview of our framework's architecture highlights its significant potential to boost the development of MLOps (e.g., data collection, preparation, and unified access to integrated data). In this section, we present three use cases that demonstrate how to carry out more complicated MLOps steps using our framework. These use cases demonstrate the ability to utilize VisionKG for composing visual datasets with unified access and taxonomy through SPARQL queries, automating training and testing pipelines, and expediting the development of robust visual recognition systems. VisionKG's features enable users to efficiently manage data from multiple sources, reduce overheads, and enhance the efficiency and reliability of machine learning models. Due to space constraints, more detailed features and tutorials about VisionKG can be found in our GitHub repository\footnote{https://github.com/cqels/vision}.
\subsection{Composing Visual Datasets with a Unified Taxonomy and SPARQL}\label{Composite Visual Dataset}

% Images provide rich set of visual information and features at a relatively low cost of acquisition and annotation~\cite{}. The emergence of numerous computer vision datasets has been promoting the continuous development of computer vision. Although models have made steady improvements regarding their performance on individual datasets, they are typically limited to specific domains and target categories~\cite{kalogeiton2016analysing}. For example, for object detection, the MS-COCO dataset focuses on common objects in natural environments and consists of 80 categories~\cite{lin2014microsoft}, whereas the BDD dataset mainly targets driving scenarios from the real-world and only contains 10 annotated target categories~\cite{yu2020bdd100k}. Accordingly, models, which are specific to a certain public benchmark~\cite{deng2009imagenet}~\cite{kuznetsova2020open}, are often trained and evaluated on their focused target dataset and scenario with restricted categories. This leads to a number of problems , such as the challenges of rare instances, imbalanced datasets, and domain shift. As a consequence state-of-the-art methods perform worse on one dataset than on another~\cite{hoffman2018cycada}. 

Data often comes in a variety of structures and schemas, and there is a need for consolidation of this information in a unified approach. Efficient data management with expressive query functionalities plays a pivotal role in MLOps. However, data from heterogeneous sources with inconsistent formats presents numerous challenges~\cite{estiri2019federated,renggli2021data} that must be addressed to ensure the efficiency and reliability of machine learning models under development. Additionally, the quality and consistency of data and unified access to data are paramount in developing visual recognition systems.

As discussed in Section~\ref{Sec:VisionKG_FAIR} and ~\ref{sec:visionkg}, VisionKG is %a unified data model powered by Resource Description Framework (RDF) based on knowledge graph. To make data accessible in a unified manner, it provides a query interface with SPARQL. The SPARQL query language provides users the ability to describe queries using RDF statements and access the desired data in a unified way, no matter of heterogeneous sources or inconsistent formats of images and annotations. In this way, VisionKG can be used to 
is equipped with SPARQL engine allowing developers to programmatically build a composite dataset (from diverse sources with different annotated formats) to significantly reduce considerable effort in data preparation phase in MLOps. 
For instance, as demonstrated in Figure~\ref{fig:UC1}\textbf{(c)}, users can query for images containing \verb|{car}| from MS-COCO\cite{lin2014microsoft} and \verb|{Sedan}| from UD-DETRACK\cite{wen2020ua} dataset, even though they have far different annotated formats (i.e., MS-COCO is in JSON and UA-DETRAC is in XML format). Furthermore, benefiting from the Semantic Enrichment Reasonder described in Section~\ref{subsec:vkg_overview} and integrated knowledge bases (e.g. WordNet~\cite{Miller:1995}),  users can query for images containing \verb|{person}| from MS-COCO, KITTI, and Visual Genome~\cite{krishna2017visual} (due to distinct taxonomies, in source datasets, \verb|{person}| are annotated as \verb|{pedestrian}| and \verb|{man}| in KITTI and Visual Genome, respectively) using a simple query (Figure~\ref{fig:fair}~\textcircled{\raisebox{-1pt}{3}}) rather than a more complex query (Figure~\ref{fig:fair}~\textcircled{\raisebox{-1pt}{1}}) that covers all possible cases: \verb|{pedestrian}| in KITTI or \verb|{man}| in Visual Genome. 

Thanks to the semantic interoperability (cf. Section~\ref{sec:inteop}) of interlinked annotations across diverse label spaces, % under a shared semantic understanding,
users can create datasets from various sources with relevant definitions as desired. Along with the enrichment of semantic relationships, VisionKG provides users with composite visual datasets in a cost-efficient and data-centric manner and hence boosts the data streaming in MLOps. \textcolor{red}{[Jicheng: can you give an example?]}

% To address this problem, users may need to improve the model performance based on model-centric methods, such as extensively tuning model parameters according to various scenarios, which is a time-consuming and labor-intensive task. VisionKG alleviates this problem by enabling users to query images with categories of similar definitions or with the same hyponym as shown in Figure~\ref{fig:UC1}\textbf{(c)}: For instance, both \verb|{car}| and \verb|{sedan}| are subclasses of \verb|{vehicle}|, thus the more general term can be used easily or both terms can be used interchangeably. Additionally, VisionKG leverages knowledge and facts from Wikidata~\cite{Wilkinson:2016} and WordNet~\cite{Miller:1995}, enabling dynamic prompts during the dataset construction process based on information from knowledge bases. For example, users can construct a dataset that includes the category \verb|{person}| from various taxonomies or domains. In this scenario, users can query the desired category \verb|{person}| from one of their target datasets, such as the MS-COCO dataset, and VisionKG will then provide prompts indicating that the KITTI and VisualGenome datasets include the categories \verb|{pedestrian}| and \verb|{man}| as these categories define persons, too. Thus users benefit from interlinked annotations across diverse label spaces under a shared semantic understanding and can create a mixed dataset from various sources with relevant definitions as desired. Along with the enrichment of semantic relationships, VisionKG provides users with composite visual datasets in a cost-efficiently and data-centric manner.

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=\textwidth]{figures/UC/[ISWC23] VIsionKG_UC23_.jpg}
%     \caption{Dataflow in VisionKG. }
%     \label{fig:UC23}
% \end{figure}
% \vspace{-8mm}
% VisionKG leverages the knowledge graph and WordNet to effectively link various datasets. By interconnecting labels across diverse spaces, VisionKG provides a common vocabulary for built-in datasets, enabling an efficient search for annotated images across multiple public datasets. This capability is particularly useful for users who need images of a specific class or scene across multiple public datasets for their learning pipelines. For instance, researchers who need to train an object detection model to perceive traffic objects on the road may require multi-source datasets, such as COCO, Objects365, Open Images Dataset, or Waymo. However, the taxonomies used in these datasets may not be compatible, such as "Car" in the COCO dataset being marked as "Van" in Objects365. VisionKG addresses this challenge by integrating different taxonomies based on WordNet Domains Hierarchy~\cite{bentivogli2004revising} and provides powerful functionalities for efficiently exploring and analyzing large-scale computer vision datasets by interconnecting labels across diverse spaces with a common vocabulary.
% What we could sell:
% \vspace{-2mm}
% \begin{enumerate}
%     \item user would like to query one categories \textbf{car}, \textbf{pedestrian} or supercategories \textbf{CAR} and \textbf{PEDESTRIAN} from multiple datasets (COCO, OID, Objects365)
%     \item for a category from multiple datasets(similar to figure 1), if it exists in one datasets, we will use it, if not, we could use its similar category to replace it (e.g. \textbf{person}$\xrightarrow{}$\textbf{pedestrian})
%     \item for a supercategory, we could return all its related categories from queried datasets (e.g. $\{car, van\} \in $\textbf{CAR})
% \end{enumerate}
% \textbf{UC3. Analyzing the robustness of DNNs under samples from semantic/visual similarities via VisionKG,later. (Anh and Jicheng)}
% Beyond interlinking labels across label spaces under shared semantic understanding and the common vocabulary for diverse datasets, VisionKG can also be leveraged for evaluating the robustness of deep neural networks (DNNs) under samples with semantic/visual similarities. VisionKG is also capable to link and integrate various samples based on semantic/visual similarity search and can help researchers identify and address potential biases and limitations in their models. By using VisionKG to generate datasets with semantic/visual similarities, researchers can evaluate the robustness of their models to variations in label spaces and on a wider range of data and improve their performance on new and diverse data.
% What we could sell:
% \vspace{-2mm}
% \begin{enumerate}
%     \item user query samples based on semantic similarity
%     \item user query samples based on visual similarity
%     \item both semantic and visual similarity
% \end{enumerate}
% \vspace{5mm}
% \textbf{UC3. Leveraging VisionKG for Training and Evaluation of Computer Vision Models.(Anh and Jicheng)} 
% \vspace{-15mm}

\subsection{Automating Training and Testing Pipelines} \label{subsec:auto_training}

One of the primary goals of MLOps is to automate the training and testing pipelines to accelerate the development and deployment of ML models~\cite{alla2021mlops}. Automated workflows enable rapid iteration and experimentation, avoiding the time-consuming process during the model development for both researchers and developers. However, despite the advancements of MLOps in increased productivity and reproducibility of experiments, there are also some limitations remain in current MLOps tools (e.g., Kubeflow~\cite{bisong2019kubeflow} and MLflow~\cite{alla2021mlops} ), such as limited support for complex data types and multi-modal data (e.g., images, videos, and audios). Besides, integrating these MLOps tools with existing diverse data infrastructures can be challenging and require significant effort.

As described in Section~\ref{sec:explorer}, powered by SPARQL, VisionKG supports automated end-to-end pipelines for visual tasks. Users can start a training pipeline by writing queries to compose composite visual datasets. As demonstrated in Figure~\ref{fig:pipelines_from_SPARQL}\circled{\textbf{a}}, users can query images and annotations with a few lines of SPARQL query to use RDF-based description to get desired data, such as images containing box-level annotations of \verb|{Sedan}|, \verb|{Car}|, and \verb|{Car, Van}| from UA-DETRAC~\cite{wen2020ua}, MS-COCO\cite{lin2014microsoft} and KITTI~\cite{geiger2013vision}. In combination with current popular frameworks (e.g., Pytorch, TensorFlow) or toolboxes (e.g., MMDetection~\cite{chen2019mmdetection}, Detectron2~\cite{wu2019detectron2}), users can further utilize the retrieved data to construct their learning pipelines in just a few lines of Python code without extra effort, as Figure~\ref{fig:pipelines_from_SPARQL}\circled{\textbf{b}} demonstrated. Users need to define solely the model they want to use and the hyperparameters they want to set.

Additionally, benefiting from the built-in models and Evaluator described in Section~\ref{subsec:vkg_overview}, users can use provided frontend interface from VisionKG to execute inferences and visualize those results to gain a quick overview of the data quality and insights about the potential model for specific scenarios, as Figure~\ref{fig:pipelines_from_SPARQL}\circled{\textbf{c}} demonstrated. On the other hand, users can also test the model performance, which is trained and provided by themselves, using data retrieved from VisionKG. This feature supports to enhance the model performance with data from different domains retrieved in VisionKG. 

These features significantly reduce the workload during data collection, preparation, pre-processing, verification, and model selection for MLOps. Due to the space limit, more features about automated pipelines powered by VisionKG can be found in our tutorials.

% Efficient data management with expressive query functionalities play a pivotal role in automating training and testing pipelines for MLOps. However, managing data from multiple sources presents numerous challenges that must be addressed to ensure the efficiency and reliability of machine learning models under development. The difficulties arising from handling data from diverse sources can be assessed from various perspectives, including data integration, completeness, consistency, heterogeneity, and timeliness~\cite{}. Integrating data from heterogeneous sources is a complex and time-consuming process. Data often comes in a variety of formats, structures, and schemas, necessitating the consolidation of this information into a unified format. Additionally, the quality and consistency of data are paramount in developing robust machine-learning models.

% With our VisionKG framework users can initiate a training pipeline by writing a SPARQL query to retrieve the desired images and labels. As shown in Figure 5(b) and described in Sec3.2, users can query images with box-level annotations such as \verb|Sedan_detrack|, \verb|Car_coco|, \verb|Van_kitti|, and \verb|Car_coco|. After VisionKG returns image URLs and annotations in JSON format, users can further utilize the retrieved data to construct their learning pipelines using PyTorch, TensorFlow, or other downstream toolboxes like mmdetection or Detectron2. Additionally, VisionKG provides training configurations for constructing training pipelines with these popular tools. As illustrated in Figure 5(c), users can initiate a training pipeline with VisionKG in just a few lines of Python code, significantly reducing the workload during data preparation and pre-processing. Users can then select the model and define detailed configurations for training, such as learning scheduler, batch size, and learning epochs.

% Moreover, VisionKG also supports pipeline testing. Currently, domain shift poses a significant challenge when transferring a model trained on source domain data to a target domain, despite the existence of domain adaptation methods. To test the model's performance across different domains, users can employ SPARQL to access VisionKG's integrated data, further validating the model's performance on various domain datasets. This process provides potential insights for enhancing the model's performance in different domains.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=\textwidth]{figures/UC/Semkg-Vision-scenario.jpg}
    \caption{Construct CV Pipelines Employing VisionKG. }
    \label{fig:pipelines_from_SPARQL}
\end{figure}


\subsection{Robust Visual Learning over Diverse Data-Sources}

The increasing demand for robust visual learning systems has led to the need for efficient MLOps practices to handle large-scale heterogeneous data, maintain data quality, and ensure seamless integration between data streamlining and model development. Moreover, a robust learning system should perform consistently well under varying conditions, such as invariance to viewpoint and scale, stable performance under instance occlusion, and robustness to illumination changes. However, many existing visual datasets are specifically designed and curated for particular tasks, often resulting in a limited distribution of image data applicable only in narrowly defined situations~\cite{paullada2021data}. This not only imposes unnecessary burdens when developing robust visual recognition systems but also introduces biases within learning systems and constrains the robustness of visual recognition systems. 

As discussed in Section~\ref{Composite Visual Dataset} and ~\ref{subsec:auto_training}, users can use VisionKG to compose datasets across interlinked data sources and semantic-rich knowledge bases and automatically build training and testing pipelines starting from SPARQL queries. This paves the way to support the construction of robust learning systems exploiting features from VisionKG. For instance,  when users want to develop a robust object detector, besides bounding boxes and annotated categories, other environmental situations should also be considered and incorporated as prior knowledge to boost the robustness of trained detectors, such as weather and illumination conditions. Using VisionKG, as demonstrated in Figure~\ref{fig:UC1}\textbf{(b)}, users can query for images with diverse conditions, such as images containing \verb|{Car}| under \verb|{rainy}| weather condition and captured during {night} time. Additionally, users can explore fruitful visual features from VisionKG as desired. This potential can assist users in evaluating the capability of domain transfer of models (e.g., if a detector trained on KITTI\cite{geiger2013vision} is also robust to detect \verb|{Car}| in \verb|{snow}| weather condition) or handle rare categories in one dataset (e.g., query for a composite dataset containing specific categories which are rare in the source dataset to address it).

These features reduce the bias arising from unrelated samples and also enables users to construct scenario-specific datasets covering rich semantics in a convenient fashion. Besides, in this way, it allows the users to build robust training pipelines in both data- and model-centric manners.

% Many existing visual datasets are specifically designed and curated for particular tasks, often resulting in a limited distribution of image data applicable only in narrowly defined situations~\cite{paullada2021data}.  This not only imposes unnecessary burdens when developing robust visual recognition systems but also introduces biases within learning systems and constrains the potential of data-centric artificial intelligence. In order to demonstrate the training process of robust learning systems through a data-centric approach, we introduce a use case involving the construction of training pipelines based on the composite dataset detailed in Sections~\ref{Exploring Visual Datasets via SPARQL} and \ref{Composite Visual Dataset}. VisionKG facilitates the initialization of a training pipeline, commencing with the composition of SPARQL queries to obtain the desired images and annotations. This encompasses advanced configurations, such as merging training data with shared hyponyms (e.g., \verb|{man}| or \verb|{person}|) from datasets with multiple sources and incorporating training data under adverse weather conditions (e.g., \verb|{snow}| or \verb|{rainy}|).

% Furthermore, to establish a robust visual recognition system tailored to specific use cases and applications, our framework seamlessly integrates data acquired via VisionKG with high-performance visual recognition toolboxes, including timm~\cite{rw2019timm}, OpenMMLab~\cite{mmdetection}, Detectron2~\cite{wu2019detectron2}, and Torchvision~\cite{torchvision2016}, as demonstrated in the dataflow of VisionKG depicted in Figure~\ref{fig:UC23}. This capability empowers users to create customized datasets from scratch, compatible with a variety of tasks, and subsequently initialize a trainer or evaluator upon visual and statistical verification of the retrieved dataset. Additionally, users can mix their self-provided data with datasets retrieved through VisionKG. This functionality expeditiously augments the model's robustness, addressing the distinct requirements of users and ultimately enhancing the resilience and robustness of visual recognition systems across multiple sources with diverse features.
% To enhance the training process of the robust learning system in a data-centric manner, we present a use case of the construction of training pipelines based on the mixed dataset based on Sec.\ref{Exploring Visual Datasets via SPARQL} and Sec.\ref{Composite Visual Dataset}. VisionKG enable users to initialize a training pipeline starting from writing SPARQL queries to retrieve desired images and annotations. This includes advanced settings such as merging training data with the same hyponym, like \{man\} or \{person\} from multiple sources datasets; and training data under adverse weather conditions, like \{snow\} or \{rainy\}. Moreover, to develop a robust visual recognition system to meet the specific use scenarios and applications, our framework seamlessly integrates data retrieved via VisionKG's API with downstream, high-performance visual recognition toolboxes such as timm~\cite{rw2019timm}, OpenMMLab~\cite{mmdetection}, Detectron2~\cite{wu2019detectron2}, and Torchvision~\cite{torchvision2016}, as the dataflow of VisionKG shown in Figure \ref{fig:UC23}. It empowers users to construct customized datasets from scratch, which is compatible with various applications, and then initialize a trainer or evaluator after verifying the retrieved dataset visually and statistically. Additionally, users also can train on their self-provided datasets and assess the trained models using datasets retrieved through VisionKG. This feature conveniently improves the model's robustness tailored to the unique needs of users and ultimately enhances the robustness of vision systems under multiple sources with diverse features.
% VisionKG also benefits to build training pipelines and evaluation models on multiple- or single-source datasets with closed or open domains. For example, researchers may need to build a training pipeline for object detection that utilizes both COCO and Open Images datasets. VisionKG can simplify this process by providing a unified interface for searching and retrieving images and annotations from these datasets, enabling researchers to efficiently build their training pipeline. Similarly, VisionKG can be used to build evaluation models for datasets with closed or open domains. Besides official annotated ground truth from source datasets, VisionKG also provides open-domain annotations, e.g. weather conditions, timeOfDay. By leveraging the capabilities for linking and integrating various sources and annotations based on knowledge graphs, VisionKG enables researchers to build unified and robust image recognition models that are able to handle variations in label spaces and achieve contextualize understanding.
% What we could sell:
% \vspace{-2mm}
% \begin{enumerate}
%     \item wide range of pseudo-labels beyond official annotations
%     \item pseudo contextual information(e.g weather condition, timeOfDay)
%     \item we need to design some vocabularies for them
% \end{enumerate}
% \vspace{5mm}

% \textbf{(Danh and Jicheng)Potentials of Vision Knowledge Graph in managing (Computer Vision) datasets and models: towards a high quality(Quantity, Versatility, and Scalability) dataset(model) platform.}
